Robust Relationship Between Mid-latitudes CAPE and Moist Static Energy in Present and Future Simulations

Convective available potential energy (CAPE), a metric associated with severe weather, is expected to increase with warming. Under the most widely-accepted theory, developed for strongly convective regimes, mean CAPE should rise following the Clausius-Clapeyron (C-C) relationship at 6-7%/K. We show here that although the magnitude of CAPE change in high-resolution model output is only slightly underestimated with simple theories, it is insufficient to describe the distributional changes, which has a down-sloping structure and is crucial for impact assessment. A more appropriate framework for understanding CAPE changes uses the tight correlation between CAPE and moist static energy (MSE) surplus. Atmospheric profiles develop appreciable CAPE only when MSE surplus becomes positive; beyond this point, CAPE increases as $\sim$25% of the rise in MSE surplus. Because this relationship is robust across climate states, changes in future CAPE distributions can be well-captured by a simple scaling of present-day data using only three parameters.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
